Mid-attribute speaker generation using optimal-transport-based interpolation of Gaussian mixture models

In this paper, we propose a method for intermediating multiple speakers' attributes and diversifying their voice characteristics in ``speaker generation,'' an emerging task that aims to synthesize a nonexistent speaker's naturally sounding voice. The conventional TacoSpawn-based speaker generation method represents the distributions of speaker embeddings by Gaussian mixture models (GMMs) conditioned with speaker attributes. Although this method enables the sampling of various speakers from the speaker-attribute-aware GMMs, it is not yet clear whether the learned distributions can represent speakers with an intermediate attribute (i.e., mid-attribute). To this end, we propose an optimal-transport-based method that interpolates the learned GMMs to generate nonexistent speakers with mid-attribute (e.g., gender-neutral) voices. We empirically validate our method and evaluate the naturalness of synthetic speech and the controllability of two speaker attributes: gender and language fluency. The evaluation results show that our method can control the generated speakers' attributes by a continuous scalar value without statistically significant degradation of speech naturalness.

==> fig/partitioning.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp3796101352946567] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (69.92,37.88) -- (329.92,37.88) -- (329.92,49.88) -- (69.92,49.88) -- cycle ;
%Shape: Rectangle [id:dp4918154254803251] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.54 ] (69.92,66.88) -- (170.92,66.88) -- (170.92,76.88) -- (69.92,76.88) -- cycle ;
%Shape: Rectangle [id:dp1263454580490353] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.56 ] (149.92,76.88) -- (260.92,76.88) -- (260.92,86.88) -- (149.92,86.88) -- cycle ;
%Shape: Rectangle [id:dp8775963547119923] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=0.55 ] (240.92,86.88) -- (329.92,86.88) -- (329.92,96.88) -- (240.92,96.88) -- cycle ;
%Straight Lines [id:da7856899965101948] 
\draw  [dash pattern={on 6pt off 2.25pt}]  (69.92,27.88) -- (69.92,114.88) ;
%Straight Lines [id:da33561458894717244] 
\draw  [dash pattern={on 6pt off 2.25pt}]  (160.92,44.88) -- (160.92,114.88) ;
%Straight Lines [id:da5346896577295797] 
\draw  [dash pattern={on 6pt off 2.25pt}]  (250.92,43.88) -- (250.92,114.88) ;
%Straight Lines [id:da5540802931101504] 
\draw    (71.92,104.88) -- (158.92,104.88) ;
\draw [shift={(160.92,104.88)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(69.92,104.88)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da15822088877530105] 
\draw    (253.92,104.88) -- (328.92,104.88) ;
\draw [shift={(330.92,104.88)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(251.92,104.88)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da653467356994818] 
\draw    (162.92,104.88) -- (249.92,104.88) ;
\draw [shift={(251.92,104.88)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(160.92,104.88)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da21017878435256443] 
\draw  [dash pattern={on 6pt off 2.25pt}]  (329.92,27.88) -- (329.92,114.88) ;
%Straight Lines [id:da640194301012043] 
\draw    (213.92,29.88) -- (327.92,29.88) ;
\draw [shift={(329.92,29.88)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da33763840313286453] 
\draw    (177.92,28.88) -- (71.92,28.88) ;
\draw [shift={(69.92,28.88)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da24706518655532705] 
\draw    (255.92,68.88) .. controls (256.88,49.58) and (266.23,56.36) .. (283.06,59.55) ;
\draw [shift={(284.92,59.88)}, rotate = 189.46] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da10966678071540714] 
\draw    (250,69) -- (260.92,68.88) ;
\draw [shift={(260.92,68.88)}, rotate = 539.39] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;

% Text Node
\draw (104,108) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{cut}}$};
% Text Node
\draw (281,107) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{last}}$};
% Text Node
\draw (194,107) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{cut}}$};
% Text Node
\draw (187,20) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{full}}$};
% Text Node
\draw (286,53) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle l_{\text{overlap}}$};


\end{tikzpicture}


==> tab/corr.tex <==
\begin{table}[t]
    \centering
    \caption{Correlation between weights(0-1) for each attribute and each subjective evaluation item.}
    \footnotesize
    \begin{tabular}{c|c c c c}
        & [m, Ja] & [m, En] & [f, Ja] & [f, En] \\
        \hline
        Gender & 0.447677 & 0.577762 & -0.551532 & -0.473907\\
        Nativeness &0.379056 & -0.374874 & 0.221033 & -0.225216
    \end{tabular}
    \label{tab:corr}
    \vspace{-4mm}
\end{table}

==> tab/mos.tex <==
\begin{table}[t]
    \centering
    \caption{Mean and standard deviation of naturalness for each attribute speaker corresponding to the weights for[[male, Japanese], [male, English], [female, Japanese], [female, English]].}
    \footnotesize
    \begin{tabular}{c|c  c|c  c|c}
        weight&naturalness&weight&naturalness&weight&naturalness\\
        \hline
        {[0, 0, 0, 1]} &$3.15 \pm 0.372$& {[0, 0.5, 0, 0.5]} &$3.03 \pm 0.444$& {[0, 1, 0, 0]}&$2.92 \pm 0.535	$ \\
        {[0, 0, 0.5, 0.5]} &$3.41 \pm 0.416$& {[0.25, 0.25, 0.25, 0.25]} &$3.36 \pm 0.374$& {[0.5, 0.5, 0, 0]} &$3.35 \pm 0.491$ \\
        {[0, 0, 1, 0]} &$3.07 \pm 0.551$& {[0.5, 0, 0.5, 0]} &$3.17 \pm 0.542$& {[1, 0, 0, 0]} &$3.35 \pm 0.421$
    \end{tabular}
    \label{tab:mos}
    \vspace{-4mm}
\end{table}

==> takamichi_memo.tex <==
\section{Takamichi's memo (ato de kesu)}
    \subsection{Tacospawn}
        \begin{align}
            p_{\theta}\pt{\Vec{s} | c} = \sum\limits_{k=1}^{K} \alpha_k\pt{c} p_k\pt{\Vec{s}|c},
        \end{align}
    where $\theta$ is a model parameter set of the encoder. $\Vec{s}$ is a $D$-dimensional speaker embedding vector, $c$ is a speaker attribute. $K$ is the number of mixtures. $\alpha_k$ and $p_{k}\pt{\Vec{s}|c} = \Normal{\Vec{s}; \Vec{\mu}_k\pt{c}, \diag{\Vec{\sigma}_k^2\pt{c}}}$ are the mixture weight and the Gaussian distribution of the $k$th mixture, respectively. $\Vec{\mu}_k$ and $...$  $\alpha_k$, $\Vec{\mu}_k$, $...$ are functions of $\theta$ but we omit to notate for clear notation.

    \subsection{TTS model with speaker attribute encoder}
    \vspace{-1mm} 
    We use multi-speaker TTS model with TacoSpawn~\cite{stanton2022speaker}-based speaker attribute encoder. The TTS model and encoder are trained as in the TacoSpawn paper. At inference, the TTS models predicts speech features conditioned by a phoneme sequence $\Vec{x}$ and a speaker embedding vector $\Vec{s}$. The encoder encodes speaker attribute $c$ to form a GMM $p\pt{\Vec{s}|c}$ to sample $\Vec{s}$. Assuming the speaker attribute takes each of $L$ kinds of values, $\left\{c_l|l=1,\cdots,L\right\}$, we form a different GMM $p\pt{\Vec{s}|c_l}$ from each $c_l$ and have $L$ GMMs in total, where the $l$th GMM is
        \begin{align}
            p\pt{\Vec{s}|c_l}   &= \sum\limits_{k=1}^{K} \alpha_{l,k} p_{l,k}\pt{\Vec{s}}, \\
            p_{l,k}\pt{\Vec{s}} &= \Normal{\Vec{s}; \Vec{\mu}_{l,k}, \Vec{\sigma}_{l,k}},
        \end{align}
    where $\alpha_{l,k}, \Vec{\mu}...$ are xxx of the $k$th mixture of the $l$th GMM.
    From these GMMs, we form xxx.
    
    \subsection{Speaker mixing}
    \subsubsection{Barycenter of Gaussian distributions: Prelimiary}
    Before interpolating $L$ GMMs, we describe the simplest case: interpolation of $L$ Gaussian distributions. Given $L$ Gaussian distributions $\left\{\Normal{\Vec{\mu}_l, \Vec{\Sigma}_l}| l=1,2,\cdots,L\right\}$ and the , the barycenter is also given as the Gaussian distribution $\Normal{\Vec{\mu}', \Vec{\sigma}'}$. The cost function is the Wassersten distance $W_2$. The objective to estimate $\Vec{\mu}', \Vec{\sigma}'$ is
        \begin{align}
            \Argmin_{\Vec{\mu}', \Vec{\sigma}'}\sum\limits_{l}\lambda_l
                W_2\pt{\Normal{\Vec{\mu}', \Vec{\sigma}'}, \Normal{\Vec{\mu}_l, \Vec{\sigma}_l}},
        \end{align}
    and is solved as 
        \begin{align}
            \Vec{\mu}' = \sum\limits_{l}\lambda_l \Vec{\mu}_l, \;\;
            \Vec{\sigma}' = \sum\limits_{l} \lambda_l^2 \Vec{\sigma}_l 
        \end{align}
    where $\leftarrow$ is the iterative update.

    \subsubsection{Barycenter of speaker space GMMs}
    Given $L$ $K$-mixture GMMs, the barycenter is given as a $K^L$-mixture GMM
        \begin{align}
            \sum\limits_{m=1}^{K^L} \alpha_{m}' \Normal{\Vec{\mu}'_{m} , \Vec{\sigma}'_{m}}
        \end{align}
    $\alpha_m', \Vec{\mu}_m'...$ are estimated by solving
        \begin{align}
            \min_{\pi_{l,k,m}} \sum\limits_{l}\sum\limits_{k}\sum\limits_{m} 
                \lambda_l \pi_{l,k,m} W_2\pt{\Normal{\Vec{\mu}'_m, \Vec{\sigma}'_m}, \Normal{\Vec{\mu}_{l,k}, \Vec{\sigma}_{l,k}}},
        \end{align}
    under
        \begin{align}
            \sum\limits_{m} \pi_{l,k,m} &= \alpha_{l,k} \\
            \sum\limits_{k} \pi_{1,k,m} &= \pi_{2,k,m} = \cdots = \pi_{L,k,m}.
        \end{align}
    Solving Eq. (xx), $\alpha_m$ is given as
        \begin{align}
            \alpha_m' = \sum\limits_{k} \pi_{l,k,m}
        \end{align}
